The Axion-Instanton Weak Gravity Conjecture and Scalar Fields

We study the Weak Gravity Conjecture in the presence of scalar fields. The Weak Gravity Conjecture is a consistency condition for a theory of quantum gravity asserting that for a U(1) gauge field, there is a particle charged under this field whose mass is bounded by its charge. It was extended to a statement about any canonical pair of (p - 1)-dimensional object and p-form coupling to it, in particular to axion-instanton pairs. The gauge-scalar Weak Gravity Conjecture is a modification of this bound that includes scalar interactions. We propose a similar extension to cases where scalar fields are present for the axion-instanton Weak Gravity Conjecture and provide evidence from Type IIA supergravity.

==> Layout/Nomenclature.tex <==
\renewcommand*{\nomprefix}{}
% Mathematics

\nomenclature[E]{$\operatorname{End}(E)$}{Endomorphism bundle of vector bundle $E$.}
\nomenclature[Gamma]{$\Gamma(E)$}{Set of all sections of a bundle $E$. Sections of $TM$ are called \emph{vector fields}.}

\nomenclature[id]{$\operatorname{id}$}{Identity map.}
\nomenclature[TM1]{$TM$}{Tangent bundle of a manifold $M$.}
\nomenclature[TM2]{$T^*M$}{Cotangent bundle of a manifold $M$.}
\nomenclature[V]{$V^\mathbb{C}$}{Complexification of a vector space $V$.}

\nomenclature[J1]{$\mathcal{J}$}{Almost complex structure of an even-dimensional differentiable manifold.}
\nomenclature[W1]{$\Omega^{r,s}$(M)}{The set $\Gamma(\Lambda^{r,s}M)$ of $(r,s)$-forms on $M$.}
\nomenclature[W2]{$\Omega$}{The non-vanishing holomorphic $n$-form on a Calabi-Yau $n$-fold.}
\nomenclature[J2]{$J$}{K\"ahler form of a Hermitian manifold.}
\nomenclature[Harm]{$\operatorname{Harm}^{r,s}(M)$}{Set of $\bar{\partial}$-harmonic $(r,s)$-forms on $M$.}
\nomenclature[H]{$H^{r,s}(M)$}{Dolbeault cohomology group.}
\nomenclature[h]{$h^{r,s}$}{Hodge number.}
\nomenclature[b]{$b^p$}{Betti number.}

% More on moduli
\nomenclature[a]{$\{\alpha_\ha,\beta^{\hat b}\}$}{Real basis of $H^3(Y) = H^{3,0}(Y)\oplus H^{2,1}(Y)\oplus H^{1,2}(Y)\oplus H^{0,3}(Y)$}
\nomenclature[A]{$\{\mathcal{B}_\ha,\mathcal{A}^{\hat b}\}$}{Basis of three-cycles for homology group corresponding to $H^3(Y)$.}
% Type II

\nomenclature[H1]{$\hat H_3, \hat F_2,...$}{Three-form, two-form etc. in ten dimensions.}
\nomenclature[H2]{$H_3, F_2,...$}{Forms in four dimensions.}

\printnomenclature[2.1cm]


==> Sections/WGCforAxions.tex <==
\section{A Weak Gravity Conjecture for Axions}
